Power Bundle Adjustment for Large-Scale 3D Reconstruction

We introduce Power Bundle Adjustment as an expansion type algorithm for solving large-scale bundle adjustment problems. It is based on the power series expansion of the inverse Schur complement and constitutes a new family of solvers that we call inverse expansion methods. We theoretically justify the use of power series and we prove the convergence of our approach. Using the real-world BAL dataset we show that the proposed solver challenges the state-of-the-art iterative methods and significantly accelerates the solution of the normal equation, even for reaching a very high accuracy. This easy-to-implement solver can also complement a recently presented distributed bundle adjustment framework. We demonstrate that employing the proposed Power Bundle Adjustment as a sub-problem solver significantly improves speed and accuracy of the distributed optimization.

==> CVPR PoBA-2/problem_size.tex <==
&\multicolumn{1}{c}{cameras}&\multicolumn{1}{c}{landmarks}&\multicolumn{1}{c}{observations} \\
\midrule
ladybug-49&49&7,766&31,812\\%
ladybug-73&73&11,022&46,091\\%
ladybug-138&138&19,867&85,184\\%
ladybug-318&318&41,616&179,883\\%
ladybug-372&372&47,410&204,434\\%
ladybug-412&412&52,202&224,205\\%
ladybug-460&460&56,799&241,842\\%
ladybug-539&539&65,208&277,238\\%
ladybug-598&598&69,193&304,108\\%
ladybug-646&646&73,541&327,199\\%
ladybug-707&707&78,410&349,753\\%
ladybug-783&783&84,384&376,835\\%
ladybug-810&810&88,754&393,557\\%
ladybug-856&856&93,284&415,551\\%
ladybug-885&885&97,410&434,681\\%
ladybug-931&931&102,633&457,231\\%
ladybug-969&969&105,759&474,396\\%
ladybug-1064&1,064&113,589&509,982\\%
ladybug-1118&1,118&118,316&528,693\\%
ladybug-1152&1,152&122,200&545,584\\%
ladybug-1197&1,197&126,257&563,496\\%
ladybug-1235&1,235&129,562&576,045\\%
ladybug-1266&1,266&132,521&587,701\\%
ladybug-1340&1,340&137,003&612,344\\%
ladybug-1469&1,469&145,116&641,383\\%
ladybug-1514&1,514&147,235&651,217\\%
ladybug-1587&1,587&150,760&663,019\\%
ladybug-1642&1,642&153,735&670,999\\%
ladybug-1695&1,695&155,621&676,317\\%
ladybug-1723&1,723&156,410&678,421\\%
\midrule
&\multicolumn{1}{c}{cameras}&\multicolumn{1}{c}{landmarks}&\multicolumn{1}{c}{observations} \\
\midrule
trafalgar-21&21&11,315&36,455\\%
trafalgar-39&39&18,060&63,551\\%
trafalgar-50&50&20,431&73,967\\%
trafalgar-126&126&40,037&148,117\\%
trafalgar-138&138&44,033&165,688\\%
trafalgar-161&161&48,126&181,861\\%
trafalgar-170&170&49,267&185,604\\%
trafalgar-174&174&50,489&188,598\\%
trafalgar-193&193&53,101&196,315\\%
trafalgar-201&201&54,427&199,727\\%
trafalgar-206&206&54,562&200,504\\%
trafalgar-215&215&55,910&203,991\\%
trafalgar-225&225&57,665&208,411\\%
trafalgar-257&257&65,131&225,698\\%
\midrule
&\multicolumn{1}{c}{cameras}&\multicolumn{1}{c}{landmarks}&\multicolumn{1}{c}{observations} \\
\midrule
dubrovnik-16&16&22,106&83,718\\%
dubrovnik-88&88&64,298&383,937\\%
dubrovnik-135&135&90,642&552,949\\%
dubrovnik-142&142&93,602&565,223\\%
dubrovnik-150&150&95,821&567,738\\%
dubrovnik-161&161&103,832&591,343\\%
dubrovnik-173&173&111,908&633,894\\%
dubrovnik-182&182&116,770&668,030\\%
dubrovnik-202&202&132,796&750,977\\%
dubrovnik-237&237&154,414&857,656\\%
dubrovnik-253&253&163,691&898,485\\%
dubrovnik-262&262&169,354&919,020\\%
dubrovnik-273&273&176,305&942,302\\%
dubrovnik-287&287&182,023&970,624\\%
dubrovnik-308&308&195,089&1,044,529\\%
dubrovnik-356&356&226,729&1,254,598\\%
\midrule
&\multicolumn{1}{c}{cameras}&\multicolumn{1}{c}{landmarks}&\multicolumn{1}{c}{observations} \\
\midrule
venice-52&52&64,053&347,173\\%
venice-89&89&110,973&562,976\\%
venice-245&245&197,919&1,087,436\\%
venice-427&427&309,567&1,695,237\\%
venice-744&744&542,742&3,054,949\\%
venice-951&951&707,453&3,744,975\\%
venice-1102&1,102&779,640&4,048,424\\%
venice-1158&1,158&802,093&4,126,104\\%
venice-1184&1,184&815,761&4,174,654\\%
venice-1238&1,238&842,712&4,286,111\\%
venice-1288&1,288&865,630&4,378,614\\%
venice-1350&1,350&893,894&4,512,735\\%
venice-1408&1,408&911,407&4,630,139\\%
venice-1425&1,425&916,072&4,652,920\\%
venice-1473&1,473&929,522&4,701,478\\%
venice-1490&1,490&934,449&4,717,420\\%
venice-1521&1,521&938,727&4,734,634\\%
venice-1544&1,544&941,585&4,745,797\\%
venice-1638&1,638&975,980&4,952,422\\%
venice-1666&1,666&983,088&4,982,752\\%
venice-1672&1,672&986,140&4,995,719\\%
venice-1681&1,681&982,593&4,962,448\\%
venice-1682&1,682&982,446&4,960,627\\%
venice-1684&1,684&982,447&4,961,337\\%
venice-1695&1,695&983,867&4,966,552\\%
venice-1696&1,696&983,994&4,966,505\\%
venice-1706&1,706&984,707&4,970,241\\%
venice-1776&1,776&993,087&4,997,468\\%
venice-1778&1,778&993,101&4,997,555\\%
\midrule
&\multicolumn{1}{c}{cameras}&\multicolumn{1}{c}{landmarks}&\multicolumn{1}{c}{observations} \\
\midrule
final-93&93&61,203&287,451\\%
final-394&394&100,368&534,408\\%
final-871&871&527,480&2,785,016\\%
final-961&961&187,103&1,692,975\\%
final-1936&1,936&649,672&5,213,731\\%
final-3068&3,068&310,846&1,653,045\\%
final-4585&4,585&1,324,548&9,124,880\\%
final-13682&13,682&4,455,575&28,973,703\\%


